On Mini-Batch Training with Varying Length Time Series

In real-world time series recognition applications, it is possible to have data with varying length patterns. However, when using artificial neural networks (ANN), it is standard practice to use fixed-sized mini-batches. To do this, time series data with varying lengths are typically normalized so that all the patterns are the same length. Normally, this is done using zero padding or truncation without much consideration. We propose a novel method of normalizing the lengths of the time series in a dataset by exploiting the dynamic matching ability of Dynamic Time Warping (DTW). In this way, the time series lengths in a dataset can be set to a fixed size while maintaining features typical to the dataset. In the experiments, all 11 datasets with varying length time series from the 2018 UCR Time Series Archive are used. We evaluate the proposed method by comparing it with 18 other length normalization methods on a Convolutional Neural Network (CNN), a Long-Short Term Memory network (LSTM), and a Bidirectional LSTM (BLSTM).

==> trash.tex <==

\begin{table*}[!t]
% \renewcommand{\arraystretch}{1.1}
    \caption{Test Accuracy (\%) Using 1D VGG (Average of Five Trainings)}
    \label{tab:results_vgg}
    \centering
    \begin{tabular}{lccccccccccc|c}
    \hline
     & \multicolumn{11}{c}{Datasets} &  \\ 
    Method & AGWX & AGWY & AGWZ & GMAD1 & GMAD2 & GMAD3 & GPZ1 & GPZ2 & PGWZ & PLAID & SGWZ & Ave. \\ 
    \hline
    0 Pad (R) & 68.3 & 66.7 & 57.8 & 71.8 & 53.6 & 42.8 & 89.1 & 84.8 & 71.3 & 49.3 & 73.3 & 66.2 \\
    0 Pad (L) & & & & & & & & & & & & \\
    0 Pad (O) & & & & & & & & & & & & \\
    E. Pad (R) & & & & & & & & & & & & \\
    E. Pad (L) & & & & & & & & & & & & \\
    E. Pad (O) & & & & & & & & & & & & \\
    Trunc. (R) & & & & & & & & & & & & \\
    Trunc. (L) & & & & & & & & & & & & \\
    Trunc. (O) & & & & & & & & & & & & \\
    Stretch & & & & & & & & & & & & \\
    STRP~\cite{iwana2021an} & & & & & & & & & & & & \\
    Rand.~\cite{iwana2021an} & & & & & & & & & & & & \\
    Zoom~\cite{iwana2021an} & & & & & & & & & & & & \\
    None & & & & & & & & & & & & \\
    Proposed & & & & & & & & & & & & \\
    \hline
    \end{tabular}
\end{table*}
\begin{table*}[!t]
% \renewcommand{\arraystretch}{1.1}
    \caption{Test Accuracy (\%) Using LSTM (Average of Five Trainings)}
    \label{tab:results_lstm}
    \centering
    \begin{tabular}{lccccccccccc|c}
    \hline
     & \multicolumn{11}{c}{Datasets} &  \\ 
    Method & AGWX & AGWY & AGWZ & GMAD1 & GMAD2 & GMAD3 & GPZ1 & GPZ2 & PGWZ & PLAID & SGWZ & Ave. \\ 
    \hline
    0 Pad (R) & 68.3 & 66.7 & 57.8 & 71.8 & 53.6 & 42.8 & 89.1 & 84.8 & 71.3 & 49.3 & 73.3 & 66.2 \\
    0 Pad (L) & & & & & & & & & & & & \\
    0 Pad (O) & & & & & & & & & & & & \\
    E. Pad (R) & & & & & & & & & & & & \\
    E. Pad (L) & & & & & & & & & & & & \\
    E. Pad (O) & & & & & & & & & & & & \\
    Trunc. (R) & & & & & & & & & & & & \\
    Trunc. (L) & & & & & & & & & & & & \\
    Trunc. (O) & & & & & & & & & & & & \\
    Stretch & & & & & & & & & & & & \\
    STRP~\cite{iwana2021an} & & & & & & & & & & & & \\
    Rand.~\cite{iwana2021an} & & & & & & & & & & & & \\
    Zoom~\cite{iwana2021an} & & & & & & & & & & & & \\
    None & & & & & & & & & & & & \\
    Proposed & & & & & & & & & & & & \\
    \hline
    \end{tabular}
\end{table*}

\begin{table*}[!t]
% \renewcommand{\arraystretch}{1.1}
    \caption{Test Accuracy (\%) Using BLSTM (Average of Five Trainings)}
    \label{tab:results_blstm}
    \centering
    \begin{tabular}{lccccccccccc|c}
    \hline
     & \multicolumn{11}{c}{Datasets} &  \\ 
    Method & AGWX & AGWY & AGWZ & GMAD1 & GMAD2 & GMAD3 & GPZ1 & GPZ2 & PGWZ & PLAID & SGWZ & Ave. \\ 
    \hline
    0 Pad (R) & 68.3 & 66.7 & 57.8 & 71.8 & 53.6 & 42.8 & 89.1 & 84.8 & 71.3 & 49.3 & 73.3 & 66.2 \\
    0 Pad (L) & & & & & & & & & & & & \\
    0 Pad (O) & & & & & & & & & & & & \\
    E. Pad (R) & & & & & & & & & & & & \\
    E. Pad (L) & & & & & & & & & & & & \\
    E. Pad (O) & & & & & & & & & & & & \\
    Trunc. (R) & & & & & & & & & & & & \\
    Trunc. (L) & & & & & & & & & & & & \\
    Trunc. (O) & & & & & & & & & & & & \\
    Stretch & & & & & & & & & & & & \\
    STRP~\cite{iwana2021an} & & & & & & & & & & & & \\
    Rand.~\cite{iwana2021an} & & & & & & & & & & & & \\
    Zoom~\cite{iwana2021an} & & & & & & & & & & & & \\
    None & & & & & & & & & & & & \\
    Proposed & & & & & & & & & & & & \\
    \hline
    \end{tabular}
\end{table*}

\begin{table}[!t]
% \renewcommand{\arraystretch}{1.1}
    \caption{Comparison Between the Datasets}
    \label{tab:properties}
    \centering
    \begin{tabular}{lccc}
    \hline
    Dataset &  Min. Len. & Max. Len. & Ave. Len.  \\ \hline
    AllGestWiiX  & 11 & 385& 124.9$\pm$65.9 \\
    AllGestWiiY  & 8 & 369 & 128.6$\pm$69.6\\
    AllGestWiiZ  & 33 & 326 & 125.5$\pm$66.3\\
    GestMidAirD1 & 80 & 360  & 166.5$\pm$63.8\\
    GestMidAirD2 & 80 & 360 & 166.5$\pm$63.8 \\
    GestMidAirD3 & 80 & 360 & 166.5$\pm$63.8 \\
    GestPebbleZ1 & 115 & 455 & 233.7$\pm$83.2 \\
    GestPebbleZ2 & 100 & 455 & 223.5$\pm$88.7 \\
    PickGestWiiZ & 29 & 361 & 145.9$\pm$78.1 \\
    PLAID & 100 & 1344 & 323.8$\pm$143.8 \\
    ShakGestWiiZ & 41 & 385 & 171.9$\pm$87.9 \\
    \hline
    \end{tabular}
\end{table}


    Zero Pad (Post) & 66.2$\pm$13.6 & 21.6$\pm$14.8 & 42.6$\pm$17.0 \\
    Zero Pad (Pre) & 62.7$\pm$13.8 & 46.6$\pm$21.1 & 52.5$\pm$17.1 \\
    Zero Pad (Outer) & 66.4$\pm$14.7 & 21.0$\pm$18.1 & 16.6$\pm$9.5 \\
    Edge Pad (Post) & 63.3$\pm$16.1 & 26.7$\pm$9.8 & 37.6$\pm$12.7 \\
    Edge Pad (Pre) & 60.6$\pm$14.8 & 36.5$\pm$15.9 & 50.1$\pm$19.4 \\
    Edge Pad (Outer) & 63.5$\pm$16.8 & 27.5$\pm$11.5 & 33.9$\pm$9.2 \\
    Truncate (Post) & 35.8$\pm$13.4 & 30.3$\pm$13.6 & 31.9$\pm$11.6 \\
    Truncate (Pre) & 38.5$\pm$17.1 & 35.5$\pm$19.7 & 37.4$\pm$18.7 \\
    Truncate (Outer) & 41.7$\pm$20.2 & 37.5$\pm$23.1 & 39.2$\pm$21.7 \\
    Interpolation & 57.4$\pm$22.5 & 41.2$\pm$20.5 & 46.0$\pm$12.3 \\
    Zero Pad (Mid)~\cite{Lopez_del_Rio_2020} &  &  &  \\
    STRP Pad~\cite{Lopez_del_Rio_2020} & 65.3$\pm$16.9 & 41.5$\pm$19.0 & 46.0$\pm$12.3 \\
    Random Pad~\cite{Lopez_del_Rio_2020} & 57.6$\pm$22.8 & 39.1$\pm$14.3 & 40.9$\pm$12.7 \\
    Zoom Pad~\cite{Lopez_del_Rio_2020} & 38.5$\pm$20.8 & 31.8$\pm$19.5 & 50.5$\pm$16.0 \\
    None ($B=1$) & 38.5$\pm$24.4 & 31.8$\pm$12.3 &  \\
    
    
    
\begin{table}[!t]
% \renewcommand{\arraystretch}{1.1}
    \caption{Effect of $\alpha$ and Class-wise (CW) Prototypes. Mean Test Accuracy (\%) of the 11 Datasets Using the Median of Five Trained Models }
    \label{tab:classwise}
    \centering
    \begin{tabular}{lccc}
    \hline
     & \multicolumn{3}{c}{Model} \\
    Method & 1D VGG & LSTM & BLSTM \\ \hline
    $\alpha=0.0$ & 63.86 & 53.74 & 56.21 \\
    $\alpha=0.1$ & 60.31 & 51.81 & 53.19 \\
    $\alpha=0.2$ & 61.68 & 54.82 & 55.00 \\
    $\alpha=0.3$ & 57.94 & 46.25 & 55.27 \\
    $\alpha=0.4$ & 60.17 & 50.82 & 46.73 \\
    $\alpha=0.5$ & 61.47 & 47.42 & 51.80 \\
    $\alpha=0.6$ & 58.10 & 46.24 & 50.07 \\
    $\alpha=0.7$ & 55.42 & 41.45 & 46.44 \\
    $\alpha=0.8$ & 54.06 & 34.60 & 45.67 \\
    $\alpha=0.9$ & 55.15 & 35.82 & 42.98 \\
    $\alpha=0.1$, CW & 61.31 & 52.35 & 54.91 \\
    $\alpha=0.2$, CW & 58.17 & 49.14 & 57.62 \\
    $\alpha=0.3$, CW & 60.28 & 49.94 & 54.03 \\
    $\alpha=0.4$, CW & 59.34 & 51.39 & 54.16 \\
    $\alpha=0.5$, CW & 58.82 & 48.94 & 51.75 \\
    $\alpha=0.6$, CW & 56.67 & 44.37 & 51.34 \\
    $\alpha=0.7$, CW & 55.38 & 43.96 & 44.59 \\
    $\alpha=0.8$, CW & 55.64 & 39.06 & 43.59 \\
    $\alpha=0.9$, CW & 55.13 & 36.22 & 42.90 \\
    \hline
    \end{tabular}
\end{table}
